Active Information Acquisition for Linear Optimization

We consider partially-specified optimization problems where the goal is to actively, but efficiently, acquire missing information about the problem in order to solve it. An algorithm designer wishes to solve a linear program (LP), $\max \mathbf{c}^T \mathbf{x}$ s.t. $\mathbf{A}\mathbf{x} \leq \mathbf{b}, \mathbf{x} \ge \mathbf{0}$, but does not initially know some of the parameters. The algorithm can iteratively choose an unknown parameter and gather information in the form of a noisy sample centered at the parameter's (unknown) value. The goal is to find an approximately feasible and optimal solution to the underlying LP with high probability while drawing a small number of samples. We focus on two cases. (1) When the parameters $\mathbf{c}$ of the objective are initially unknown, we take an information-theoretic approach and give roughly matching upper and lower sample complexity bounds, with an (inefficient) successive-elimination algorithm. (2) When the parameters $\mathbf{b}$ of the constraints are initially unknown, we propose an efficient algorithm combining techniques from the ellipsoid method for LP and confidence-bound approaches from bandit algorithms. The algorithm adaptively gathers information about constraints only as needed in order to make progress. We give sample complexity bounds for the algorithm and demonstrate its improvement over a naive approach via simulation.

==> related.tex <==
\subsection{Related work}

%If no additional information about the constraint parameters is available, the company will have to do its best with prior knowledge and assumptions.
%In this case, it has available techniques from a variety of literatures including stochastic programming~\citep{heyman2003stochastic,neely2010stochastic}, chance-constrained programming~\citep{ben2009robust}, and robust optimization~\citep{ben2009robust,bertsimas2004robust}.
%
%In this work, we suppose the solver of the optimization problem, e.g. the company, can \emph{actively gather data} about these constraints in order to find a better solution.
%For instance, the delivery company can choose to send an observer to a particular road segment to observe the travel time on that segment for that particular day.
%There are two challenges: (1) it is costly to gather this data; (2) each data point is only a \emph{noisy sample} of the underlying true constraint.
%For instance, the delivery company wishes to minimize expected travel time, but the observed travel time on any given day may be random, centered around the true mean that the company cares about, but with variance.
%The company will need to inspect that edge of the graph several different times, i.e. send an observer on several different days, to gain confidence about its average travel time.
%
%One approach would be to gather data about all parameters, e.g. send observers to every road segment for many days, until high confidence about all parameters is achieved.
%Then one can solve the optimization problem to high accuracy because all parameters are known to high accuracy.
%However, this is very costly in terms of resources, as measured by the total number of data points that must be gathered.
%There may be many road segments, but only a few will ultimately be important to the solution.
%Instead, we suppose that the company can actively choose at each time to sample an additional data point about any particular constraint, e.g. choose each day where to send an observer. 
%How should the company choose which data points to sample so as to solve the optimization problem to within high accuracy and confidence, while minimizing the total amount of data that must be collected?
%
%We formalize this question for the problem of solving general linear programs (described in Section \ref{sec:problem}) and propose an algorithm to solve it.
%We suppose that the parameters of some constraints are initially unknown and that, at each time, the algorithm can draw a ``sample'' of one of these parameters, which is distributed with mean equal to the true parameter, but with some variance.
%The goal of the algorithm is to parsimoniously draw sampled data about the important/relevant constraints in order to gradually solve the linear program with high probability and to high accuracy.
%Our main result is a bound on the number of samples it needs to draw as a function of the features of the problem.
%We will also present some simulation results.
%
%Our algorithm combines two main ideas: the ellipsoid method for solving linear programs, and \emph{multi-armed bandit} techniques for gathering data and making decisions based on that data.
%The ellipsoid algorithm makes progress by taking a current proposed solution, finding a violated constraint, and using it to ``cut'' the space of feasible solutions.
%Its efficiency guarantees are that it needs to cut using relatively few total constraints to find a solution.
%But how to find a violated constraint, or check that none are violated, using a small amount of data?
%Our approach is to use bandit techniques, specifically relating confidence bounds to the number of samples obtained so far.
%In some cases, only a few samples are enough to be confident that a constraint is or is not violated; in others, many are needed.
%Confidence bounds allow us to quantify and distinguish these cases.
%
%This approach allows us to theoretically bound the number of data points drawn by our algorithm as a function of the parameters of the problem.
%In simulations on generated linear programs, it performs quite closely to a hypothetical benchmark algorithm that knows which are the binding constraints in advance.
%In other words, the algorithm spends very few resources (in terms of number of data points) on parameters that do not end up mattering in the optimal solution, as compared to those that do.
%

\paragraph{Related work: overview.}
The setting considered in this paper, active information acquisition for optimization, is related at a high level to a large number of lines of work that deal with optimization and uncertainty.
However, most of them solve a different conceptual problem, failing to model either the optimization aspect or the active aspect. At a technical level, some works are relatively close to our model, but do not provide useful solutions to the model of linear AIAO studied here.

\paragraph{Related work: Theoretical computer science and machine learning.}
Much work in \emph{active learning} considers acquiring data points iteratively with a goal of low sample complexity \citet{balcan2006agnostic,balcan2007margin,castro2008minimax}.The key difference to AIAO is between \emph{data} and \emph{parameters}.
In learning, the goal is to minimize the average or expectation of some loss function over a distribution of data points.
Other than its likelihood, each data point plays the same role in the problem.
Here, the focus is on how much information about each of various parameters is necessary to solve a structured optimization problem to a desired level of accuracy.
In other words, the key question here, which is how much an optimization algorithm needs to know about the parameters of the problem it is solving, does not apply in active learning.

Broadly related is recent work on \emph{optimization from samples} \citet{balkanski2016power}, which considers the sample complexity of a two-stage process: (1) draw some number of i.i.d. data points; (2) optimize some loss function or submodular function on the data.
In that setting, the algorithm sees a number of input-output pairs of the function, randomly distributed, and must eventually choose a particular input to optimize the function.
Therefore, it is quite different from our setting in both important ways: (1) the information collected are data points (and evaluations), as in ML above, rather than parameters as in our problem; (2) (so far) it is not active, but acquires information in a batch.

%\bo{TODO! Combinatorial pure exploration!}
A line of work that is closely related to our problem is the study of \emph{combinatorial pure exploration} (CPE) problem, where a learner collects samples of unknown parameters of an objective function to identify the optimal member in a solution set. The problem was first proposed in \cite{chen2014combinatorial}, and subsequently studied by~\cite{gabillon2016improved, chen2016combinatorial, chen2016pure, lijie17}.  CPE only considers combinatorial optimization problems whose solution set contains only binary vectors of length $n$. A recent work by~\cite{lijie17} extended CPE to a \emph{General-Sampling} problem by allowing general solution sets. Our unknown-$\V{c}$ problem can be fitted into the setting of General-Sampling. Nevertheless, our algorithm for unknown-$\V{c}$ leverages the structure of LP and hence has better sample complexity performance than directly treating it as a General-Sampling problem.
%, which is guaranteed no more than $\ln(1/\Delta)$ times the lower bound, whereas their algorithm can have an additional $n^2$ factor compared to the lower bound. 
The General-Sampling problem does not encompass all AIAO settings, e.g., our unknown-$\V{b}$ case.

\paragraph{Related work: artificial intelligence.}

%\yc{For the related work in AI, maybe we want to be explicit on what relates to the unknown c setting and what to the unknown b setting.}

Several existing lines of work in the artificial intelligence literature, deal with actively acquiring information about parameters of an optimization problem in order to solve it.
Preference elicitation~\citep{braziunas2006computational,blum2004preference} typically focuses on acquiring information about parameters of the \emph{objective} by querying a user about his preferences, this is similar to our goal for the unknown-$\V{c}$ setting. But often the existing literatures do not analyze an active information acquisition setting; neither do they analyze the sample complexity. \bo{(? not quite sure)}%\yc{The previous sentence needs to be changed. I think it comes from our previous draft. So, what are the differences between our unknown c case and the preference elicitation literature? I guess they don't consider sample complexity? It's important to make it clear.} \yc{This seems to be only related to our unknown b case.}
Relevant to our unknown-$\V{b}$ case, for more combinatorial problems, the constraint acquisition literature~\citep{oconnell2002strategies,bessiere2015constraint} is closer to our problem in some respects, as it posits an optimization problem with unknown constraints that must be learned via interactive querying.

We emphasize that a central feature of the model in this paper is \emph{noisy observations}: the observations of the algorithm are only noisy samples of a true underlying constraint.
The key challenge is to choose how many repeated samples of each parameter to draw so as to gain confidence in using or discarding its constraint.
This aspect of the problem is not to our knowledge present in preference elicitation or model/constraint acquisition.
This also differs from the literatures on stochastic programming~\citep{heyman2003stochastic,neely2010stochastic}, chance-constrained programming~\citep{ben2009robust}, and robust optimization~\citep{ben2009robust,bertsimas2004robust}.

%\yc{I think we can safely remove the following discussion on crowdsourcing. They are not that relevant. Maybe we can keep the waze example somewhere in the intro?}[commented out.]
%
%Our model is motivated by the practice of actively acquiring information from people in crowdsourcing systems \citep{howe2006rise}, especially in crowdsensing \citep{reddy2010recruitment,ganti2011mobile,koutsopoulos2013optimal,chon2012automatically,gao2014jigsaw}, where noisy information can be elicited quickly and provide valuable information for many applications.
%Recently, crowdsensing has become a popular solution to companies or organization for collecting information from crowds conveniently.
%
%
%The idea of using crowdsourcing or crowdsensing has been used for information collection for different goals. For example, in \cite{abernethy2015low}, data are actively purchased from crowd workers for running online learning algorithms. In \cite{gao2013online}, the similar idea of querying data from crowdsourcing has been implemented within the context of online decision making. \cite{chon2012automatically} uses the idea of crowdsensing to characterize places based on data collected from smartphones. Another example is to use crowdsensing data to help with indoor plan reconstruction [\cite{gao2014jigsaw}].
%
%
%

